A projection algorithm on measures sets

We consider the problem of projecting a probability measure $\pi$ on a set $\mathcal{M}\_N$ of Radon measures. The projection is defined as a solution of the following variational problem:\begin{equation*}\inf\_{\mu\in \mathcal{M}\_N} \|h\star (\mu - \pi)\|\_2^2,\end{equation*}where $h\in L^2(\Omega)$ is a kernel, $\Omega\subset \R^d$ and $\star$ denotes the convolution operator.To motivate and illustrate our study, we show that this problem arises naturally in various practical image rendering problems such as stippling (representing an image with $N$ dots) or continuous line drawing (representing an image with a continuous line).We provide a necessary and sufficient condition on the sequence $(\mathcal{M}\_N)\_{N\in \N}$ that ensures weak convergence of the projections $(\mu^*\_N)\_{N\in \N}$ to $\pi$.We then provide a numerical algorithm to solve a discretized version of the problem and show several illustrations related to computer-assisted synthesis of artistic paintings/drawings.

==> Halftoning.tex <==
In this section and the next, we show how the general results proposed previously allow solving the practical problems of stippling and continuous line drawing. 
We first focus on the case of N-point measures $\mathcal{M}(\Omega^N)$ defined in equation \ref{eq:NPointMeasures}.
This setting is the standard one considered for probability quantization. As mentioned earlier, it has many applications including image stippling.

Using the results derived in Section \ref{sec:math}, we obtain the following guarantees.
\begin{theorem}\label{thm:consistence_N-point}
Let $\mathcal{M}_N=\mathcal{M}(\Omega^N)$ denote the sequence of N-point measures.
Then there exists solutions $\mu^*_N$ to the projection problem \eqref{eq:projection}.

Moreover, for any Lipschitz kernel $h\in \mathcal{C}(\Omega)$:
\begin{itemize}
\item[i)] $\mu_N^*\underset{N\to \infty}{\rightharpoonup} \pi$.
\item[ii)] $\mathcal{N}_h(\mu^*_N - \pi) = \mathcal{O}\left(  N^{-\frac{1}{d}} \right).$
\end{itemize}
\end{theorem}
\begin{proof}
In the case of N-point measures, the projection problem \eqref{eq:projection} can be recast as \eqref{eq:halftone_problem}.
Let $p=(p_1,\cdots,p_N) \in \Omega^N$. 
The mapping $p\mapsto \left\|h\star \left(\pi - \frac{1}{N}\sum_{i=1}^N \delta_{p_i}\right) \right\|_2^2$ is continuous. 
Problem \eqref{eq:halftone_problem} therefore consists of minimizing a finite dimensional continuous function over a compact set. 
The existence of a solution follows. We let $\mu^*_N$ denote the associated measure. 

In order to prove i) and ii), it suffices to evaluate the bound $\delta_N$ defined in \eqref{eq:defdeltaN}.
To this end, for any given $\pi$, we construct an explicit sequence of measures $\mu_0, \dots, \mu_N$, the last of which is an $N$-point measure approximating $\pi$.

Note that $\T^d$ can be thought of as the unit cube $[0,1)^d$. 
It may therefore be partitioned in $C^d$ smaller cubes of edge length $1/C$ with $C=\lfloor N^{1/d}\rfloor$.
We let $(\omega_i)_{1\leq i \leq C^d}$ denote the small cubes and $x_i$ denote their center.
We assume that the cubes are ordered in such a way that $\omega_i$ and $\omega_{i+1}$ are contiguous.

We define $\displaystyle \mu_0 = \sum_{i=1}^{C^d} \pi(\omega_i)\delta_{x_i}$.
The measure $\mu_0$ satisfies
\begin{align*}
    W_1(\pi, \mu_0)       &  \leq \sup_i \text{Diameter}(\omega _i) \\
                          &  = \mathcal{O}(N^{-1/d}), \\
\end{align*}
but is not an $N$-point measure since $N \pi(\omega_i)$ is not an integer. 

To obtain an $N$-point measure, we recursively build $\mu_l$ as follows:
\begin{align*}
    \mu_l(\{x_l\}) & = \frac{1}{N} \left\lfloor{ N \mu_{l-1}(\{x_l\}) }\right\rfloor, \\
    \mu_l(\{x_{l+1}\}) & = \mu_{l-1}(\{x_{l+1}, x_l\}) 
    - \frac{1}{N} \left\lfloor{N \mu_{l-1}(\{x_l\}) }\right\rfloor, \\
                        \mu_l(\{x_i\}) & = \mu_{l-1}(\{x_i\}) \text{\quad if } i\neq l, l+1.    
\end{align*}
Notice that $N\mu_l(x_i)$ is an integer for all $i\leq l$. Therefore $\mu_N$ is an $N$-point measure.
Moreover:
\begin{align*}
    W_1(\mu_l, \mu_{l+1}) & \leq \frac{1}{N} \|x_l - x_{l+1}\| \\
                          & \leq \mathcal{O}(N^{-1 - 1/d}).
\end{align*}
Since the transportation distance is a distance, we have the triangle inequality.
Therefore:
\begin{align*}
    W_1(\pi, \mu_N)       & \leq W_1(\pi, \mu_0) + \sum_{l=1}^N W_1(\mu_{l-1}, \mu_l), \\
                          &  =   \mathcal{O}(N^{-1/d}) + N \mathcal{O}(N^{-1 - 1/d}) \\
                          &  = \mathcal{O}(N^{-1/d}).     
\end{align*}
\end{proof}

The Algorithm \eqref{algo:Npoint} can be applied directly and provide an approximate projection.
To finish this paragraph, let us acknowledge that consistency of problem \eqref{eq:electorhalftone} was already studied in the recent papers \cite{graf2012quadrature,fornasier2013consistency,fornasier2013consistency2}. To the best of our knowledge, Theorem \ref{thm:consistence_N-point} is stronger than existing results since it yields a convergence rate and holds true under more general assumptions.


